Layer stripping approach to reconstruct shape defects in waveguides using locally resonant frequencies

This article present a new method to reconstruct slowly varying width defects in 2D waveguides using one-side section measurements at locally resonant frequencies. At these frequencies, locally resonant modes propagate in the waveguide up to a "cut-off" position. In this particular point, the local width of the waveguide can be recovered. Given multi-frequency measurements taken on a section of the waveguide, we perform an efficient layer stripping approach to recover shape variations slice by slice. It provides an L infinite-stable method to reconstruct the width of a slowly monotonous varying waveguide. We validate this method on numerical data and discuss its limits.

==> [5] Layer stripping approach resonances /postpross1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%

\begin{axis}[%
width=5in,
height=1.2in,
at={(0in,0in)},
scale only axis,
xmin=30.9,
xmax=31.95,
xlabel={$k$},
ymin=0,
ymax=3.2,
grid=major, 
axis background/.style={fill=white},
legend style={at={(6.4in,1in)}, legend cell align=left, align=right, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
30.92	2.19015254917185\\
30.9220240480962	2.43254797463001\\
30.9240480961924	2.66126321904646\\
30.9260721442886	2.87900586838238\\
30.9280961923848	3.08768618854365\\
30.930120240481	0.147120066825315\\
30.9321442885772	0.341567449762892\\
30.9341683366733	0.530278172960853\\
30.9361923847695	0.713927556655885\\
30.9382164328657	0.893066964254796\\
30.9402404809619	1.06815375771601\\
30.9422645290581	1.23957223021296\\
30.9442885771543	1.40764928753225\\
30.9463126252505	1.57266564229235\\
30.9483366733467	1.73486455687211\\
30.9503607214429	1.89445867745578\\
30.9523847695391	2.05163498970235\\
30.9544088176353	2.2065590277204\\
30.9564328657315	2.35937831315864\\
30.9584569138277	2.51022495246343\\
30.9604809619238	2.6592176778361\\
30.96250501002	2.80646379757887\\
30.9645290581162	2.95206072365736\\
30.9665531062124	3.09609719721493\\
30.9685771543086	0.0970615897651284\\
30.9706012024048	0.238213475145695\\
30.972625250501	0.378028524547473\\
30.9746492985972	0.516569769416056\\
30.9766733466934	0.653895487167044\\
30.9786973947896	0.790059638557566\\
30.9807214428858	0.9251123567269\\
30.982745490982	1.05910033378251\\
30.9847695390782	1.19206714444265\\
30.9867935871744	1.32405351589762\\
30.9888176352705	1.45509755377109\\
30.9908416833667	1.5852350080663\\
30.9928657314629	1.71449948080453\\
30.9948897795591	1.84292260340878\\
30.9969138276553	1.97053418095574\\
30.9989378757515	2.09736232752425\\
31.0009619238477	2.22343361945135\\
31.0029859719439	2.34877321353592\\
31.0050100200401	2.47340494613716\\
31.0070340681363	2.59735141814151\\
31.0090581162325	2.72063409608388\\
31.0110821643287	2.8432733914835\\
31.0131062124249	2.96528872627106\\
31.015130260521	3.0866986034012\\
31.0171543086172	0.0659280126056778\\
31.0191783567134	0.186179101337043\\
31.0212024048096	0.305875300250126\\
31.0232264529058	0.425031989827225\\
31.025250501002	0.543663890851697\\
31.0272745490982	0.661785096905188\\
31.0292985971944	0.779409111272107\\
31.0313226452906	0.896548887951923\\
31.0333466933868	1.01321686310813\\
31.035370741483	1.12942498394166\\
31.0373947895792	1.24518473325678\\
31.0394188376754	1.36050714621874\\
31.0414428857715	1.47540284185818\\
31.0434669338677	1.58988204802147\\
31.0454909819639	1.70395462153802\\
31.0475150300601	1.8176300670687\\
31.0495390781563	1.9309175547399\\
31.0515631262525	2.04382593662424\\
31.0535871743487	2.15636375774626\\
31.0556112224449	2.26853926644649\\
31.0576352705411	2.38036043643328\\
31.0596593186373	2.49183498066807\\
31.0616833667335	2.60297036336863\\
31.0637074148297	2.71377381131107\\
31.0657314629259	2.82425232447989\\
31.067755511022	2.93441268611213\\
31.0697795591182	3.04426147217675\\
31.0718036072144	0.0122124067164364\\
31.0738276553106	0.121456981133802\\
31.0758517034068	0.23040853699265\\
31.077875751503	0.339072894807785\\
31.0798997995992	0.447455708571336\\
31.0819238476954	0.555562472517845\\
31.0839478957916	0.663398527541027\\
31.0859719438878	0.770969067283351\\
31.087995991984	0.878279143918721\\
31.0900200400802	0.985333673646901\\
31.0920440881764	1.0921374419177\\
31.0940681362725	1.19869510840029\\
31.0960921843687	1.3050112117128\\
31.0981162324649	1.41109017333652\\
31.1001402805611	1.5169362970279\\
31.1021643286573	1.62255377566261\\
31.1041883767535	1.72794669820546\\
31.1062124248497	1.83311905344578\\
31.1082364729459	1.9380747335344\\
31.1102605210421	2.04281753736168\\
31.1122845691383	2.14735117378704\\
31.1143086172345	2.25167926472599\\
31.1163326653307	2.35580534810382\\
31.1183567134269	2.45973288068224\\
31.120380761523	2.56346524076541\\
31.1224048096192	2.66700573079249\\
31.1244288577154	2.77035757982155\\
31.1264529058116	2.87352394591091\\
31.1284769539078	2.97650791791714\\
31.130501002004	3.07931251412093\\
31.1325250501002	0.0403480329274366\\
31.1345490981964	0.142802671320876\\
31.1365731462926	0.245086605271009\\
31.1385971943888	0.347202605945121\\
31.140621242485	0.449153387900445\\
31.1426452905812	0.55094161079716\\
31.1446693386774	0.652569881046702\\
31.1466933867735	0.754040753397739\\
31.1487174348697	0.855356732462702\\
31.1507414829659	0.956520274188076\\
31.1527655310621	1.05753378726998\\
31.1547895791583	1.15839963451894\\
31.1568136272545	1.25912013417496\\
31.1588376753507	1.35969756117507\\
31.1608617234469	1.46013414837653\\
31.1628857715431	1.56043208749661\\
31.1649098196393	1.66059352781933\\
31.1669338677355	1.76062057837721\\
31.1689579158317	1.8605153107063\\
31.1709819639279	1.96027975989231\\
31.1730060120241	2.05991592555607\\
31.1750300601202	2.15942577280533\\
31.1770541082164	2.25881123315549\\
31.1790781563126	2.35807420541957\\
31.1811022044088	2.45721655656927\\
31.183126252505	2.55624012256762\\
31.1851503006012	2.65514670917533\\
31.1871743486974	2.75393809273093\\
31.1891983967936	2.85261602090637\\
31.1912224448898	2.95118221343848\\
31.193246492986	3.04963836283795\\
31.1952705410822	0.00639348148635577\\
31.1972945891784	0.104634516660706\\
31.1993186372746	0.202770429633603\\
31.2013426853707	0.300802809698286\\
31.2033667334669	0.398733220205028\\
31.2053907815631	0.496563200925937\\
31.2074148296593	0.594294268869209\\
31.2094388777555	0.691927918831226\\
31.2114629258517	0.789465623931935\\
31.2134869739479	0.886908836135451\\
31.2155110220441	0.984258986754899\\
31.2175350701403	1.08151748694327\\
31.2195591182365	1.17868572817046\\
31.2215831663327	1.27576508268641\\
31.2236072144289	1.3727569039718\\
31.2256312625251	1.46966252717601\\
31.2276553106212	1.56648326954313\\
31.2296793587174	1.66322043082594\\
31.2317034068136	1.75987529368926\\
31.2337274549098	1.85644912410222\\
31.235751503006	1.95294317171948\\
31.2377755511022	2.04935867021712\\
31.2397995991984	2.14569683669333\\
31.2418236472946	2.2419588719439\\
31.2438476953908	2.3381459618635\\
31.245871743487	2.43425927783602\\
31.2478957915832	2.53029997705896\\
31.2499198396794	2.62626920285969\\
31.2519438877756	2.72216808500377\\
31.2539679358717	2.81799773999528\\
31.2559919839679	2.91375927137034\\
31.2580160320641	3.00945376998254\\
31.2600400801603	3.10508231428245\\
31.2620641282565	0.0590533169994991\\
31.2640881763527	0.154553139766922\\
31.2661122244489	0.249990171842512\\
31.2681362725451	0.345365444720471\\
31.2701603206413	0.44067997878922\\
31.2721843687375	0.535934783572639\\
31.2742084168337	0.631130857890916\\
31.2762324649299	0.726269189314255\\
31.2782565130261	0.821350754714551\\
31.2802805611222	0.916376521024787\\
31.2823046092184	1.01134744546226\\
31.2843286573146	1.10626447573809\\
31.2863527054108	1.20112855026255\\
31.288376753507	1.29594059834568\\
31.2904008016032	1.39070154039316\\
31.2924248496994	1.48541228809911\\
31.2944488977956	1.58007374463336\\
31.2964729458918	1.67468680482594\\
31.298496993988	1.76925235534689\\
31.3005210420842	1.86377127488304\\
31.3025450901804	1.95824443431064\\
31.3045691382766	2.05267269684942\\
31.3065931863727	2.14705691781453\\
31.3086172344689	2.2413979447407\\
31.3106412825651	2.33569661799644\\
31.3126653306613	2.42995377096483\\
31.3146893787575	2.52417023019706\\
31.3167134268537	2.61834681556151\\
31.3187374749499	2.71248434039163\\
31.3207615230461	2.80658361162958\\
31.3227855711423	2.90064542996869\\
31.3248096192385	2.99467058999182\\
31.3268336673347	3.08865988029748\\
31.3288577154309	0.0410214298068041\\
31.3308817635271	0.134941322260687\\
31.3329058116232	0.228827675047256\\
31.3349298597194	0.322681253699045\\
31.3369539078156	0.416502818427553\\
31.3389779559118	0.510293124230159\\
31.341002004008	0.604052920913052\\
31.3430260521042	0.697782953273578\\
31.3450501002004	0.791483961185815\\
31.3470741482966	0.885156679714846\\
31.3490981963928	0.978801839311615\\
31.351122244489	1.07242016592803\\
31.3531462925852	1.16601238112594\\
31.3551703406814	1.25957920216488\\
31.3571943887776	1.35312134186863\\
31.3592184368737	1.44663950881683\\
31.3612424849699	1.54013440762249\\
31.3632665330661	1.63360673903659\\
31.3652905811623	1.72705720004861\\
31.3673146292585	1.82048648398496\\
31.3693386773547	1.9138952806071\\
31.3713627254509	2.00728427620719\\
31.3733867735471	2.1006541537034\\
31.3754108216433	2.19400559273346\\
31.3774348697395	2.28733926974773\\
31.3794589178357	2.38065585806446\\
31.3814829659319	2.47395602759109\\
31.3835070140281	2.56724044506515\\
31.3855310621243	2.6605097743976\\
31.3875551102204	2.75376467676373\\
31.3895791583166	2.84700581068975\\
31.3916032064128	2.94023383213786\\
31.393627254509	3.03344939459105\\
31.3956513026052	3.1266531491366\\
31.3976753507014	0.0782530909593255\\
31.3996993987976	0.171435173782761\\
31.4017234468938	0.264607388411694\\
31.40374749499	0.357770377172127\\
31.4057715430862	0.4509247804015\\
31.4077955911824	0.544071236527831\\
31.4098196392786	0.637210382148684\\
31.4118436873748	0.730342852109114\\
31.4138677354709	0.82346927957947\\
31.4158917835671	0.916590296126991\\
31.4179158316633	1.00970653148821\\
31.4199398797595	1.10281861346956\\
31.4219639278557	1.1959271684703\\
31.4239879759519	1.28903282159883\\
31.4260120240481	1.38213619674893\\
31.4280360721443	1.47523791667122\\
31.4300601202405	1.5683386030505\\
31.4320841683367	1.66143887657602\\
31.4341082164329	1.75453935701777\\
31.4361322645291	1.84764066329671\\
31.4381563126253	1.94074341356043\\
31.4401803607214	2.03384822525269\\
31.4422044088176	2.12695571518876\\
31.4442284569138	2.22006649962563\\
31.44625250501	2.31318119433478\\
31.4482765531062	2.40630041467458\\
31.4503006012024	2.49942477566163\\
31.4523246492986	2.59255489204275\\
31.4543486973948	2.68569137836718\\
31.456372745491	2.77883484905794\\
31.4583967935872	2.87198591848395\\
31.4604208416834	2.96514520103191\\
31.4624448897796	3.05831331117801\\
31.4644689378758	0.0098982099704692\\
31.4664929859719	0.103085819351243\\
31.4685170340681	0.196284100205819\\
31.4705410821643	0.289493667188928\\
31.4725651302605	0.382715135408478\\
31.4745891783567	0.475949120497507\\
31.4766132264529	0.569196238687937\\
31.4786372745491	0.662457106883231\\
31.4806613226453	0.755732342732152\\
31.4826853707415	0.849022564702544\\
31.4847094188377	0.942328392155645\\
31.4867334669339	1.03565044542036\\
31.4887575150301	1.1289893458685\\
31.4907815631263	1.22234571599017\\
31.4928056112224	1.31572017946969\\
31.4948296593186	1.40911336126182\\
31.4968537074148	1.50252588766876\\
31.498877755511	1.59595838641783\\
31.5009018036072	1.68941148673905\\
31.5029258517034	1.7828858194443\\
31.5049498997996	1.87638201700629\\
31.5069739478958	1.96990071363878\\
31.508997995992	2.06344254537722\\
31.5110220440882	2.15700815016002\\
31.5130460921844	2.25059816791108\\
31.5150701402806	2.34421324062246\\
31.5170941883768	2.43785401243873\\
31.5191182364729	2.53152112974123\\
31.5211422845691	2.62521524123421\\
31.5231663326653	2.7189369980309\\
31.5251903807615	2.81268705374195\\
31.5272144288577	2.90646606443429\\
31.5292384769539	3.00027468823261\\
31.5312625250501	3.09411358584106\\
31.5332865731463	0.0463907672303456\\
31.5353106212425	0.140292206089295\\
31.5373346693387	0.234225918380641\\
31.5393587174349	0.328192576795242\\
31.5413827655311	0.422192857259756\\
31.5434068136273	0.516227439034235\\
31.5454308617234	0.610297004811652\\
31.5474549098196	0.704402240819615\\
31.5494789579158	0.798543836922189\\
31.551503006012	0.892722486724477\\
31.5535270541082	0.986938887678331\\
31.5555511022044	1.08119374118953\\
31.5575751503006	1.17548775272753\\
31.5595991983968	1.26982163193565\\
31.561623246493	1.36419609274462\\
31.5636472945892	1.45861185348705\\
31.5656713426854	1.55306963701406\\
31.5676953907816	1.64757017081415\\
31.5697194388778	1.74211418713396\\
31.5717434869739	1.83670242310169\\
31.5737675350701	1.93133562085192\\
31.5757915831663	2.02601452765364\\
31.5778156312625	2.12073989603983\\
31.5798396793587	2.2155124839407\\
31.5818637274549	2.3103330548179\\
31.5838877755511	2.40520237780302\\
31.5859118236473	2.50012122783728\\
31.5879358717435	2.59509038581559\\
31.5899599198397	2.69011063873216\\
31.5919839679359	2.78518277982971\\
31.5940080160321	2.88030760875214\\
31.5960320641283	2.97548593168305\\
31.5980561122244	3.07071856107474\\
31.6000801603206	0.024413662178091\\
31.6021042084168	0.119757368025148\\
31.604128256513	0.215157858083352\\
31.6061523046092	0.310615972788064\\
31.6081763527054	0.40613256012896\\
31.6102004008016	0.501708475831499\\
31.6122244488978	0.597344583541144\\
31.614248496994	0.693041755013049\\
31.6162725450902	0.788800870305593\\
31.6182965931864	0.884622817978432\\
31.6203206412826	0.980508495295865\\
31.6223446893788	1.07645880843443\\
31.6243687374749	1.1724746726962\\
31.6263927855711	1.26855701272667\\
31.6284168336673	1.36470676273862\\
31.6304408817635	1.46092486674149\\
31.6324649298597	1.55721227877649\\
31.6344889779559	1.65356996315753\\
31.6365130260521	1.74999889471875\\
31.6385370741483	1.84650005906857\\
31.6405611222445	1.94307445284965\\
31.6425851703407	2.03972308400709\\
31.6446092184369	2.13644697206249\\
31.6466332665331	2.23324714839627\\
31.6486573146293	2.33012465653734\\
31.6506813627255	2.42708055246094\\
31.6527054108216	2.52411590489473\\
31.6547294589178	2.62123179563336\\
31.656753507014	2.71842931986217\\
31.6587775551102	2.8157095864898\\
31.6608016032064	2.91307371849076\\
31.6628256513026	3.01052285325757\\
31.6648496993988	3.10805814296396\\
31.666873747495	0.0640881013480374\\
31.6688977955912	0.161799218456228\\
31.6709218436874	0.259600039482937\\
31.6729458917836	0.357491779062929\\
31.6749699398798	0.455475668048397\\
31.676993987976	0.553552954446065\\
31.6790180360721	0.651724903891168\\
31.6810420841683	0.749992800108135\\
31.6830661322645	0.848357945386116\\
31.6850901803607	0.946821661069738\\
31.6871142284569	1.04538528806536\\
31.6891382765531	1.1440501873649\\
31.6911623246493	1.24281774058544\\
31.6931863727455	1.3416893505281\\
31.6952104208417	1.4406664417547\\
31.6972344689379	1.53975046118471\\
31.6992585170341	1.63894287871205\\
31.7012825651303	1.73824518784342\\
31.7033066132265	1.83765890635887\\
31.7053306613226	1.93718557699519\\
31.7073547094188	2.03682676815409\\
31.709378757515	2.13658407463553\\
31.7114028056112	2.23645911839697\\
31.7134268537074	2.33645354934129\\
31.7154509018036	2.43656904613306\\
31.7174749498998	2.53680731704535\\
31.719498997996	2.637170100838\\
31.7215230460922	2.73765916766977\\
31.7235470941884	2.8382763200448\\
31.7255711422846	2.93902339379624\\
31.7275951903808	3.03990225910735\\
31.729619238477	3.14091482157379\\
31.7316432865731	0.100470369717939\\
31.7336673346693	0.201756190496631\\
31.7356913827655	0.303181648957363\\
31.7377154308617	0.404748803842011\\
31.7397394789579	0.506459755292802\\
31.7417635270541	0.608316646202532\\
31.7437875751503	0.710321663621436\\
31.7458116232465	0.812477039974212\\
31.7478356713427	0.914785053954795\\
31.7498597194389	1.01724803278736\\
31.7518837675351	1.11986835408136\\
31.7539078156313	1.22264844757277\\
31.7559318637275	1.32559079694402\\
31.7579559118236	1.42869794172721\\
31.7599799599198	1.53197247929478\\
31.762004008016	1.63541706694394\\
31.7640280561122	1.73903442407929\\
31.7660521042084	1.84282733449947\\
31.7680761523046	1.94679864879515\\
31.7701002004008	2.05095128686416\\
31.772124248497	2.15528824055132\\
31.7741482965932	2.25981257642044\\
31.7761723446894	2.36452743866787\\
31.7781963927856	2.46943605218535\\
31.7802204408818	2.57454172578267\\
31.782244488978	2.67984785558014\\
31.7842685370741	2.7853579285828\\
31.7862925851703	2.89107552644803\\
31.7883166332665	2.99700432945983\\
31.7903406813627	3.10314812072425\\
31.7923647294589	0.0679181370117412\\
31.7943887775551	0.174503687801813\\
31.7964128256513	0.281316238701148\\
31.7984368737475	0.388360031051558\\
31.8004609218437	0.495639433901996\\
31.8024849699399	0.603158949906753\\
31.8045090180361	0.710923221586423\\
31.8065330661323	0.818937037978952\\
31.8085571142285	0.927205341711979\\
31.8105811623246	1.03573323641535\\
31.8126052104208	1.14452599371586\\
31.814629258517	1.25358906222077\\
31.8166533066132	1.36292807724868\\
31.8186773547094	1.47254887058379\\
31.8207014028056	1.58245748090227\\
31.8227254509018	1.69266016493892\\
31.824749498998	1.80316340945886\\
31.8267735470942	1.91397394410879\\
31.8287975951904	2.02509875522881\\
31.8308216432866	2.13654510071617\\
31.8328456913828	2.24832052604185\\
31.834869739479	2.36043288153341\\
31.8368937875751	2.47289034105038\\
31.8389178356713	2.58570142219487\\
31.8409418837675	2.69887500821713\\
31.8429659318637	2.81242037179562\\
31.8449899799599	2.92634720089543\\
31.8470140280561	3.04066562693577\\
31.8490380761523	0.0137936019376639\\
31.8510621242485	0.128927546488306\\
31.8530861723447	0.244486465015918\\
31.8551102204409	0.360482600559074\\
31.8571342685371	0.4769288256309\\
31.8591583166333	0.593838691231852\\
31.8611823647295	0.711226481011977\\
31.8632064128257	0.829107270376056\\
31.8652304609218	0.947496991849121\\
31.867254509018	1.06641251093459\\
31.8692785571142	1.18587170928481\\
31.8713026052104	1.30589357757965\\
31.8733266533066	1.42649831992401\\
31.8753507014028	1.54770747159298\\
31.877374749499	1.66954403231097\\
31.8793987975952	1.79203261769215\\
31.8814228456914	1.91519963201917\\
31.8834468937876	2.03907346622299\\
31.8854709418838	2.16368472579561\\
31.88749498998	2.28906649446434\\
31.8895190380762	2.41525464086895\\
31.8915430861723	2.54228817730584\\
31.8935671342685	2.67020968198015\\
31.8955911823647	2.79906579934926\\
31.8976152304609	2.92890783708656\\
31.8996392785571	3.05979248096916\\
31.9016633266533	0.0501900131587298\\
31.9036873747495	0.183355997011848\\
31.9057114228457	0.317776677809153\\
31.9077354709419	0.453541253333686\\
31.9097595190381	0.590751322115754\\
31.9117835671343	0.729523590113534\\
31.9138076152305	0.869993414551832\\
31.9158316633267	1.01231953247664\\
31.9178557114228	1.15669050918259\\
31.919879759519	1.30333375328049\\
31.9219038076152	1.45252851239451\\
31.9239278557114	1.60462531060282\\
31.9259519038076	1.76007630067952\\
31.9279759519038	1.91948537744863\\
31.93	2.08369707859467\\
};
\addlegendentry{$\Phi^{-1}(u_{k,N}/q)$}

\addplot [color=mycolor2, draw=none, mark size=2.5pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
30.940612244898	0.539880947637959\\
30.9612244897959	2.49039402243656\\
30.9818367346939	1.4498606399039\\
31.0024489795918	2.26977650369783\\
31.0230612244898	0.553705315310919\\
31.0436734693878	1.20060977635086\\
31.0642857142857	2.61236017535178\\
31.0848979591837	0.581367084962613\\
31.1055102040816	1.90703132606279\\
31.1261224489796	2.86150441079381\\
31.1467346938776	0.897517295745853\\
31.1673469387755	1.66526842326826\\
31.1879591836735	2.79550671017935\\
31.2085714285714	0.491632810572444\\
31.2291836734694	1.57816202325346\\
31.2497959183673	2.56908544745527\\
31.2704081632653	0.38559971984623\\
31.2910204081633	1.46040207378812\\
31.3116326530612	2.35109628001248\\
31.3322448979592	0.224532704903801\\
31.3528571428571	1.16992263812439\\
31.3734693877551	2.06823364156024\\
31.3940816326531	3.06074520158585\\
31.414693877551	0.814761057883796\\
31.435306122449	1.76044272161634\\
31.4559183673469	2.73332959899176\\
31.4765306122449	0.501570603505193\\
31.4971428571429	1.48691854367826\\
31.5177551020408	2.44612154300959\\
31.5383673469388	0.242637765803902\\
31.5589795918367	1.24102235180531\\
31.5795918367347	2.18751300560454\\
31.6002040816327	0.017419662535147\\
31.6208163265306	1.01270318650022\\
31.6414285714286	1.96566025585254\\
31.6620408163265	2.96866467281204\\
31.6826530612245	0.821197310933091\\
31.7032653061225	1.80711873587443\\
31.7238775510204	2.84545362821195\\
31.7444897959184	0.716563978664745\\
31.7651020408163	1.76595452854668\\
31.7857142857143	2.84271420445943\\
31.8063265306122	0.772619268861543\\
31.8269387755102	1.9084652779984\\
31.8475510204082	3.04666615072753\\
31.8681632653061	1.10779066125373\\
31.8887755102041	2.35252537965933\\
31.909387755102	0.569365147271601\\
31.93	2.12425245519976\\
};
\addlegendentry{$I=50$}

\addplot [color=mycolor3, draw=none, mark size=3.5pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
30.9612244897959	2.49039402243656\\
31.0024489795918	2.26977650369783\\
31.0436734693878	1.20060977635086\\
31.0848979591837	0.581367084962614\\
31.1261224489796	2.86150441079381\\
31.1673469387755	1.66526842326826\\
31.2085714285714	0.491632810572444\\
31.2497959183673	2.56908544745526\\
31.2910204081633	1.46040207378812\\
31.3322448979592	0.224532704903801\\
31.3734693877551	2.06823364156024\\
31.414693877551	0.814761057883794\\
31.4559183673469	2.73332959899176\\
31.4971428571429	1.48691854367826\\
31.5383673469388	0.242637765803914\\
31.5795918367347	2.18751300560455\\
31.6208163265306	1.01270318650022\\
31.6620408163265	2.96866467281204\\
31.7032653061225	1.80711873587442\\
31.7444897959184	0.716563978664746\\
31.7857142857143	2.84271420445943\\
31.8269387755102	1.90846527799841\\
31.8681632653061	1.10779066125373\\
31.909387755102	0.569365147271591\\
};
\addlegendentry{$I=25$}

\addplot [color=mycolor4, draw=none, mark size=6.0pt, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
31.0024489795918	2.26977650369783\\
31.0848979591837	0.581367084962614\\
31.1673469387755	1.66526842326826\\
31.2497959183673	2.56908544745526\\
31.3322448979592	0.224532704903801\\
31.414693877551	0.814761057883794\\
31.4971428571429	1.48691854367826\\
31.5795918367347	2.18751300560455\\
31.6620408163265	2.96866467281204\\
31.7444897959184	0.716563978664746\\
31.8269387755102	1.90846527799841\\
31.909387755102	0.569365147271591\\
};
\addlegendentry{$I=13$}

\end{axis}


==> [5] Layer stripping approach resonances /postpross2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%

\begin{axis}[%
width=5in,
height=1.2in,
at={(0in,-1.7in)},
scale only axis,
xmin=30.9,
grid =major, 
xmax=31.95,
xlabel={$k$},
ymin=0,
ymax=60,
axis background/.style={fill=white},
legend style={at={(6.3in,1in)}, legend cell align=left, align=right, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2]
  table[row sep=crcr]{%
30.92	2.19015254917185\\
30.9220240480962	2.43254797463001\\
30.9240480961924	2.66126321904646\\
30.9260721442886	2.87900586838238\\
30.9280961923848	3.08768618854365\\
30.930120240481	3.28871272041511\\
30.9321442885772	3.48316010335269\\
30.9341683366733	3.67187082655065\\
30.9361923847695	3.85552021024568\\
30.9382164328657	4.03465961784459\\
30.9402404809619	4.20974641130581\\
30.9422645290581	4.38116488380275\\
30.9442885771543	4.54924194112205\\
30.9463126252505	4.71425829588214\\
30.9483366733467	4.8764572104619\\
30.9503607214429	5.03605133104557\\
30.9523847695391	5.19322764329214\\
30.9544088176353	5.34815168131019\\
30.9564328657315	5.50097096674843\\
30.9584569138277	5.65181760605323\\
30.9604809619238	5.80081033142589\\
30.96250501002	5.94805645116866\\
30.9645290581162	6.09365337724715\\
30.9665531062124	6.23768985080472\\
30.9685771543086	6.38024689694471\\
30.9706012024048	6.52139878232528\\
30.972625250501	6.66121383172706\\
30.9746492985972	6.79975507659564\\
30.9766733466934	6.93708079434663\\
30.9786973947896	7.07324494573715\\
30.9807214428858	7.20829766390649\\
30.982745490982	7.3422856409621\\
30.9847695390782	7.47525245162224\\
30.9867935871744	7.60723882307721\\
30.9888176352705	7.73828286095068\\
30.9908416833667	7.86842031524588\\
30.9928657314629	7.99768478798411\\
30.9948897795591	8.12610791058837\\
30.9969138276553	8.25371948813533\\
30.9989378757515	8.38054763470384\\
31.0009619238477	8.50661892663093\\
31.0029859719439	8.63195852071551\\
31.0050100200401	8.75659025331674\\
31.0070340681363	8.8805367253211\\
31.0090581162325	9.00381940326346\\
31.0110821643287	9.12645869866309\\
31.0131062124249	9.24847403345064\\
31.015130260521	9.36988391058078\\
31.0171543086172	9.49070597337506\\
31.0191783567134	9.61095706210642\\
31.0212024048096	9.7306532610195\\
31.0232264529058	9.8498099505966\\
31.025250501002	9.96844185162108\\
31.0272745490982	10.0865630576746\\
31.0292985971944	10.2041870720415\\
31.0313226452906	10.3213268487213\\
31.0333466933868	10.4379948238775\\
31.035370741483	10.554202944711\\
31.0373947895792	10.6699626940262\\
31.0394188376754	10.7852851069881\\
31.0414428857715	10.9001808026276\\
31.0434669338677	11.0146600087908\\
31.0454909819639	11.1287325823074\\
31.0475150300601	11.2424080278381\\
31.0495390781563	11.3556955155093\\
31.0515631262525	11.4686038973936\\
31.0535871743487	11.5811417185156\\
31.0556112224449	11.6933172272159\\
31.0576352705411	11.8051383972027\\
31.0596593186373	11.9166129414374\\
31.0616833667335	12.027748324138\\
31.0637074148297	12.1385517720805\\
31.0657314629259	12.2490302852493\\
31.067755511022	12.3591906468815\\
31.0697795591182	12.4690394329461\\
31.0718036072144	12.5785830210756\\
31.0738276553106	12.687827595493\\
31.0758517034068	12.7967791513518\\
31.077875751503	12.905443509167\\
31.0798997995992	13.0138263229305\\
31.0819238476954	13.121933086877\\
31.0839478957916	13.2297691419002\\
31.0859719438878	13.3373396816425\\
31.087995991984	13.4446497582779\\
31.0900200400802	13.5517042880061\\
31.0920440881764	13.6585080562769\\
31.0940681362725	13.7650657227595\\
31.0960921843687	13.871381826072\\
31.0981162324649	13.9774607876957\\
31.1001402805611	14.0833069113871\\
31.1021643286573	14.1889243900218\\
31.1041883767535	14.2943173125646\\
31.1062124248497	14.399489667805\\
31.1082364729459	14.5044453478936\\
31.1102605210421	14.6091881517209\\
31.1122845691383	14.7137217881462\\
31.1143086172345	14.8180498790852\\
31.1163326653307	14.922175962463\\
31.1183567134269	15.0261034950414\\
31.120380761523	15.1298358551246\\
31.1224048096192	15.2333763451517\\
31.1244288577154	15.3367281941807\\
31.1264529058116	15.4398945602701\\
31.1284769539078	15.5428785322763\\
31.130501002004	15.6456831284801\\
31.1325250501002	15.7483113008764\\
31.1345490981964	15.8507659392698\\
31.1365731462926	15.95304987322\\
31.1385971943888	16.0551658738941\\
31.140621242485	16.1571166558494\\
31.1426452905812	16.2589048787461\\
31.1446693386774	16.3605331489957\\
31.1466933867735	16.4620040213467\\
31.1487174348697	16.5633200004117\\
31.1507414829659	16.664483542137\\
31.1527655310621	16.7654970552189\\
31.1547895791583	16.8663629024679\\
31.1568136272545	16.9670834021239\\
31.1588376753507	17.067660829124\\
31.1608617234469	17.1680974163255\\
31.1628857715431	17.2683953554456\\
31.1649098196393	17.3685567957683\\
31.1669338677355	17.4685838463262\\
31.1689579158317	17.5684785786553\\
31.1709819639279	17.6682430278413\\
31.1730060120241	17.767879193505\\
31.1750300601202	17.8673890407543\\
31.1770541082164	17.9667745011045\\
31.1790781563126	18.0660374733685\\
31.1811022044088	18.1651798245182\\
31.183126252505	18.2642033905166\\
31.1851503006012	18.3631099771243\\
31.1871743486974	18.4619013606799\\
31.1891983967936	18.5605792888553\\
31.1912224448898	18.6591454813874\\
31.193246492986	18.7576016307869\\
31.1952705410822	18.8559494030251\\
31.1972945891784	18.9541904381995\\
31.1993186372746	19.0523263511724\\
31.2013426853707	19.150358731237\\
31.2033667334669	19.2482891417438\\
31.2053907815631	19.3461191224647\\
31.2074148296593	19.443850190408\\
31.2094388777555	19.54148384037\\
31.2114629258517	19.6390215454707\\
31.2134869739479	19.7364647576742\\
31.2155110220441	19.8338149082937\\
31.2175350701403	19.931073408482\\
31.2195591182365	20.0282416497092\\
31.2215831663327	20.1253210042252\\
31.2236072144289	20.2223128255106\\
31.2256312625251	20.3192184487148\\
31.2276553106212	20.4160391910819\\
31.2296793587174	20.5127763523647\\
31.2317034068136	20.609431215228\\
31.2337274549098	20.706005045641\\
31.235751503006	20.8024990932582\\
31.2377755511022	20.8989145917559\\
31.2397995991984	20.9952527582321\\
31.2418236472946	21.0915147934827\\
31.2438476953908	21.1877018834023\\
31.245871743487	21.2838151993748\\
31.2478957915832	21.3798558985977\\
31.2499198396794	21.4758251243984\\
31.2519438877756	21.5717240065425\\
31.2539679358717	21.667553661534\\
31.2559919839679	21.7633151929091\\
31.2580160320641	21.8590096915213\\
31.2600400801603	21.9546382358212\\
31.2620641282565	22.0502018921281\\
31.2640881763527	22.1457017148955\\
31.2661122244489	22.2411387469711\\
31.2681362725451	22.336514019849\\
31.2701603206413	22.4318285539178\\
31.2721843687375	22.5270833587012\\
31.2742084168337	22.6222794330195\\
31.2762324649299	22.7174177644428\\
31.2782565130261	22.8124993298431\\
31.2802805611222	22.9075250961533\\
31.2823046092184	23.0024960205908\\
31.2843286573146	23.0974130508666\\
31.2863527054108	23.1922771253911\\
31.288376753507	23.2870891734742\\
31.2904008016032	23.3818501155217\\
31.2924248496994	23.4765608632277\\
31.2944488977956	23.5712223197619\\
31.2964729458918	23.6658353799545\\
31.298496993988	23.7604009304754\\
31.3005210420842	23.8549198500116\\
31.3025450901804	23.9493930094392\\
31.3045691382766	24.043821271978\\
31.3065931863727	24.1382054929431\\
31.3086172344689	24.2325465198693\\
31.3106412825651	24.326845193125\\
31.3126653306613	24.4211023460934\\
31.3146893787575	24.5153188053256\\
31.3167134268537	24.6094953906901\\
31.3187374749499	24.7036329155202\\
31.3207615230461	24.7977321867581\\
31.3227855711423	24.8917940050972\\
31.3248096192385	24.9858191651204\\
31.3268336673347	25.079808455426\\
31.3288577154309	25.1737626585251\\
31.3308817635271	25.267682550979\\
31.3329058116232	25.3615689037656\\
31.3349298597194	25.4554224824174\\
31.3369539078156	25.5492440471459\\
31.3389779559118	25.6430343529485\\
31.341002004008	25.7367941496314\\
31.3430260521042	25.8305241819919\\
31.3450501002004	25.9242251899042\\
31.3470741482966	26.0178979084332\\
31.3490981963928	26.11154306803\\
31.351122244489	26.2051613946464\\
31.3531462925852	26.2987536098443\\
31.3551703406814	26.3923204308832\\
31.3571943887776	26.485862570587\\
31.3592184368737	26.5793807375352\\
31.3612424849699	26.6728756363408\\
31.3632665330661	26.7663479677549\\
31.3652905811623	26.859798428767\\
31.3673146292585	26.9532277127033\\
31.3693386773547	27.0466365093254\\
31.3713627254509	27.1400255049255\\
31.3733867735471	27.2333953824217\\
31.3754108216433	27.3267468214518\\
31.3774348697395	27.4200804984661\\
31.3794589178357	27.5133970867828\\
31.3814829659319	27.6066972563094\\
31.3835070140281	27.6999816737835\\
31.3855310621243	27.7932510031159\\
31.3875551102204	27.8865059054821\\
31.3895791583166	27.9797470394081\\
31.3916032064128	28.0729750608562\\
31.393627254509	28.1661906233094\\
31.3956513026052	28.2593943778549\\
31.3976753507014	28.3525869732675\\
31.3996993987976	28.4457690560909\\
31.4017234468938	28.5389412707198\\
31.40374749499	28.6321042594803\\
31.4057715430862	28.7252586627096\\
31.4077955911824	28.818405118836\\
31.4098196392786	28.9115442644568\\
31.4118436873748	29.0046767344173\\
31.4138677354709	29.0978031618876\\
31.4158917835671	29.1909241784351\\
31.4179158316633	29.2840404137963\\
31.4199398797595	29.3771524957777\\
31.4219639278557	29.4702610507784\\
31.4239879759519	29.563366703907\\
31.4260120240481	29.6564700790571\\
31.4280360721443	29.7495717989794\\
31.4300601202405	29.8426724853586\\
31.4320841683367	29.9357727588842\\
31.4341082164329	30.0288732393259\\
31.4361322645291	30.1219745456048\\
31.4381563126253	30.2150772958686\\
31.4401803607214	30.3081821075608\\
31.4422044088176	30.4012895974969\\
31.4442284569138	30.4944003819338\\
31.44625250501	30.5875150766429\\
31.4482765531062	30.6806342969827\\
31.4503006012024	30.7737586579698\\
31.4523246492986	30.8668887743509\\
31.4543486973948	30.9600252606753\\
31.456372745491	31.0531687313661\\
31.4583967935872	31.1463198007921\\
31.4604208416834	31.2394790833401\\
31.4624448897796	31.3326471934862\\
31.4644689378758	31.4258247458684\\
31.4664929859719	31.5190123552492\\
31.4685170340681	31.6122106361038\\
31.4705410821643	31.7054202030869\\
31.4725651302605	31.7986416713064\\
31.4745891783567	31.8918756563954\\
31.4766132264529	31.9851227745859\\
31.4786372745491	32.0783836427812\\
31.4806613226453	32.1716588786301\\
31.4826853707415	32.2649491006005\\
31.4847094188377	32.3582549280536\\
31.4867334669339	32.4515769813183\\
31.4887575150301	32.5449158817664\\
31.4907815631263	32.6382722518881\\
31.4928056112224	32.7316467153676\\
31.4948296593186	32.8250398971597\\
31.4968537074148	32.9184524235667\\
31.498877755511	33.0118849223158\\
31.5009018036072	33.105338022637\\
31.5029258517034	33.1988123553422\\
31.5049498997996	33.2923085529042\\
31.5069739478958	33.3858272495367\\
31.508997995992	33.4793690812752\\
31.5110220440882	33.5729346860579\\
31.5130460921844	33.666524703809\\
31.5150701402806	33.7601397765204\\
31.5170941883768	33.8537805483367\\
31.5191182364729	33.9474476656392\\
31.5211422845691	34.0411417771321\\
31.5231663326653	34.1348635339288\\
31.5251903807615	34.2286135896399\\
31.5272144288577	34.3223926003322\\
31.5292384769539	34.4162012241305\\
31.5312625250501	34.510040121739\\
31.5332865731463	34.6039099567181\\
31.5353106212425	34.697811395577\\
31.5373346693387	34.7917451078684\\
31.5393587174349	34.885711766283\\
31.5413827655311	34.9797120467475\\
31.5434068136273	35.073746628522\\
31.5454308617234	35.1678161942994\\
31.5474549098196	35.2619214303073\\
31.5494789579158	35.3560630264099\\
31.551503006012	35.4502416762122\\
31.5535270541082	35.5444580771661\\
31.5555511022044	35.6387129306773\\
31.5575751503006	35.7330069422153\\
31.5595991983968	35.8273408214234\\
31.561623246493	35.9217152822323\\
31.5636472945892	36.0161310429748\\
31.5656713426854	36.1105888265018\\
31.5676953907816	36.2050893603019\\
31.5697194388778	36.2996333766217\\
31.5717434869739	36.3942216125894\\
31.5737675350701	36.4888548103396\\
31.5757915831663	36.5835337171414\\
31.5778156312625	36.6782590855276\\
31.5798396793587	36.7730316734284\\
31.5818637274549	36.8678522443056\\
31.5838877755511	36.9627215672907\\
31.5859118236473	37.057640417325\\
31.5879358717435	37.1526095753033\\
31.5899599198397	37.2476298282199\\
31.5919839679359	37.3427019693174\\
31.5940080160321	37.4378267982399\\
31.5960320641283	37.5330051211708\\
31.5980561122244	37.6282377505625\\
31.6000801603206	37.7235255052556\\
31.6021042084168	37.8188692111027\\
31.604128256513	37.9142697011609\\
31.6061523046092	38.0097278158656\\
31.6081763527054	38.1052444032065\\
31.6102004008016	38.200820318909\\
31.6122244488978	38.2964564266187\\
31.614248496994	38.3921535980906\\
31.6162725450902	38.4879127133831\\
31.6182965931864	38.5837346610559\\
31.6203206412826	38.6796203383734\\
31.6223446893788	38.7755706515119\\
31.6243687374749	38.8715865157737\\
31.6263927855711	38.9676688558042\\
31.6284168336673	39.0638186058161\\
31.6304408817635	39.160036709819\\
31.6324649298597	39.256324121854\\
31.6344889779559	39.352681806235\\
31.6365130260521	39.4491107377963\\
31.6385370741483	39.5456119021461\\
31.6405611222445	39.6421862959272\\
31.6425851703407	39.7388349270846\\
31.6446092184369	39.83555881514\\
31.6466332665331	39.9323589914738\\
31.6486573146293	40.0292364996149\\
31.6506813627255	40.1261923955385\\
31.6527054108216	40.2232277479722\\
31.6547294589178	40.3203436387109\\
31.656753507014	40.4175411629397\\
31.6587775551102	40.5148214295673\\
31.6608016032064	40.6121855615683\\
31.6628256513026	40.7096346963351\\
31.6648496993988	40.8071699860415\\
31.666873747495	40.9047925980153\\
31.6688977955912	41.0025037151235\\
31.6709218436874	41.1003045361502\\
31.6729458917836	41.1981962757302\\
31.6749699398798	41.2961801647157\\
31.676993987976	41.3942574511134\\
31.6790180360721	41.4924294005585\\
31.6810420841683	41.5906972967754\\
31.6830661322645	41.6890624420534\\
31.6850901803607	41.787526157737\\
31.6871142284569	41.8860897847327\\
31.6891382765531	41.9847546840322\\
31.6911623246493	42.0835222372528\\
31.6931863727455	42.1823938471954\\
31.6952104208417	42.281370938422\\
31.6972344689379	42.380454957852\\
31.6992585170341	42.4796473753794\\
31.7012825651303	42.5789496845107\\
31.7033066132265	42.6783634030262\\
31.7053306613226	42.7778900736625\\
31.7073547094188	42.8775312648214\\
31.709378757515	42.9772885713028\\
31.7114028056112	43.0771636150643\\
31.7134268537074	43.1771580460086\\
31.7154509018036	43.2772735428004\\
31.7174749498998	43.3775118137127\\
31.719498997996	43.4778745975053\\
31.7215230460922	43.5783636643371\\
31.7235470941884	43.6789808167121\\
31.7255711422846	43.7797278904635\\
31.7275951903808	43.8806067557747\\
31.729619238477	43.9816193182411\\
31.7316432865731	44.082767519975\\
31.7336673346693	44.1840533407537\\
31.7356913827655	44.2854787992145\\
31.7377154308617	44.3870459540991\\
31.7397394789579	44.4887569055499\\
31.7417635270541	44.5906137964596\\
31.7437875751503	44.6926188138785\\
31.7458116232465	44.7947741902313\\
31.7478356713427	44.8970822042119\\
31.7498597194389	44.9995451830445\\
31.7518837675351	45.1021655043385\\
31.7539078156313	45.2049455978299\\
31.7559318637275	45.3078879472011\\
31.7579559118236	45.4109950919843\\
31.7599799599198	45.5142696295519\\
31.762004008016	45.617714217201\\
31.7640280561122	45.7213315743364\\
31.7660521042084	45.8251244847566\\
31.7680761523046	45.9290957990523\\
31.7701002004008	46.0332484371213\\
31.772124248497	46.1375853908084\\
31.7741482965932	46.2421097266775\\
31.7761723446894	46.346824588925\\
31.7781963927856	46.4517332024425\\
31.7802204408818	46.5568388760398\\
31.782244488978	46.6621450058372\\
31.7842685370741	46.7676550788399\\
31.7862925851703	46.8733726767051\\
31.7883166332665	46.9793014797169\\
31.7903406813627	47.0854452709814\\
31.7923647294589	47.1918079408586\\
31.7943887775551	47.2983934916487\\
31.7964128256513	47.405206042548\\
31.7984368737475	47.5122498348985\\
31.8004609218437	47.6195292377489\\
31.8024849699399	47.7270487537536\\
31.8045090180361	47.8348130254333\\
31.8065330661323	47.9428268418258\\
31.8085571142285	48.0510951455589\\
31.8105811623246	48.1596230402622\\
31.8126052104208	48.2684157975628\\
31.814629258517	48.3774788660677\\
31.8166533066132	48.4868178810956\\
31.8186773547094	48.5964386744307\\
31.8207014028056	48.7063472847492\\
31.8227254509018	48.8165499687858\\
31.824749498998	48.9270532133058\\
31.8267735470942	49.0378637479557\\
31.8287975951904	49.1489885590757\\
31.8308216432866	49.2604349045631\\
31.8328456913828	49.3722103298887\\
31.834869739479	49.4843226853803\\
31.8368937875751	49.5967801448973\\
31.8389178356713	49.7095912260418\\
31.8409418837675	49.822764812064\\
31.8429659318637	49.9363101756425\\
31.8449899799599	50.0502370047423\\
31.8470140280561	50.1645554307827\\
31.8490380761523	50.2792760593744\\
31.8510621242485	50.394410003925\\
31.8530861723447	50.5099689224526\\
31.8551102204409	50.6259650579958\\
31.8571342685371	50.7424112830676\\
31.8591583166333	50.8593211486685\\
31.8611823647295	50.9767089384487\\
31.8632064128257	51.0945897278127\\
31.8652304609218	51.2129794492858\\
31.867254509018	51.3318949683713\\
31.8692785571142	51.4513541667215\\
31.8713026052104	51.5713760350163\\
31.8733266533066	51.6919807773607\\
31.8753507014028	51.8131899290297\\
31.877374749499	51.9350264897477\\
31.8793987975952	52.0575150751288\\
31.8814228456914	52.1806820894559\\
31.8834468937876	52.3045559236597\\
31.8854709418838	52.4291671832323\\
31.88749498998	52.554548951901\\
31.8895190380762	52.6807370983056\\
31.8915430861723	52.8077706347425\\
31.8935671342685	52.9356921394168\\
31.8955911823647	53.064548256786\\
31.8976152304609	53.1943902945233\\
31.8996392785571	53.3252749384058\\
31.9016633266533	53.4572651241852\\
31.9036873747495	53.5904311080383\\
31.9057114228457	53.7248517888356\\
31.9077354709419	53.8606163643602\\
31.9097595190381	53.9978264331422\\
31.9117835671343	54.13659870114\\
31.9138076152305	54.2770685255783\\
31.9158316633267	54.4193946435031\\
31.9178557114228	54.5637656202091\\
31.919879759519	54.710408864307\\
31.9219038076152	54.859603623421\\
31.9239278557114	55.0117004216293\\
31.9259519038076	55.167151411706\\
31.9279759519038	55.3265604884751\\
31.93	55.4907721896212\\
};
\addlegendentry{$t_i^{\app}$}

\addplot [color=mycolor2, mark=o, mark options={mycolor2}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
30.940612244898	3.68147360122775\\
30.9612244897959	5.63198667602636\\
30.9818367346939	7.73304594708349\\
31.0024489795918	8.55296181087742\\
31.0230612244898	9.9784832760803\\
31.0436734693878	10.6253877371202\\
31.0642857142857	12.0371381361212\\
31.0848979591837	13.1477376993218\\
31.1055102040816	14.473401940422\\
31.1261224489796	15.427875025153\\
31.1467346938776	16.6054805636948\\
31.1673469387755	17.3732316912172\\
31.1879591836735	18.5034699781283\\
31.2085714285714	19.3411887321112\\
31.2291836734694	20.4277179447922\\
31.2497959183673	21.418641368994\\
31.2704081632653	22.3767482949748\\
31.2910204081633	23.4515506489167\\
31.3116326530612	24.342244855141\\
31.3322448979592	25.3572739336221\\
31.3528571428571	26.3026638668427\\
31.3734693877551	27.2009748702786\\
31.3940816326531	28.1934864303042\\
31.414693877551	29.0890949401919\\
31.435306122449	30.0347766039245\\
31.4559183673469	31.0076634812999\\
31.4765306122449	31.9174971394031\\
31.4971428571429	32.9028450795762\\
31.5177551020408	33.8620480789075\\
31.5383673469388	34.8001569552916\\
31.5589795918367	35.798541541293\\
31.5795918367347	36.7450321950923\\
31.6002040816327	37.7165315056127\\
31.6208163265306	38.7118150295777\\
31.6414285714286	39.6647720989301\\
31.6620408163265	40.6677765158896\\
31.6826530612245	41.6619018076004\\
31.7032653061225	42.6478232325417\\
31.7238775510204	43.6861581248793\\
31.7444897959184	44.6988611289218\\
31.7651020408163	45.7482516788038\\
31.7857142857143	46.8250113547165\\
31.8063265306122	47.8965090727084\\
31.8269387755102	49.0323550818453\\
31.8475510204082	50.1705559545744\\
31.8681632653061	51.3732731186904\\
31.8887755102041	52.618007837096\\
31.909387755102	53.9764402582981\\
31.93	55.5313275662262\\
};
\addlegendentry{$t_i$, $I=50$}

\addplot [color=mycolor3, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
30.9612244897959	2.49039402243656\\
31.0024489795918	2.26977650369783\\
31.0436734693878	4.34220242994065\\
31.0848979591837	6.8645523921422\\
31.1261224489796	9.1446897179734\\
31.1673469387755	11.0900463840376\\
31.2085714285714	13.0580034249316\\
31.2497959183673	15.1354560618144\\
31.2910204081633	17.1683653417371\\
31.3322448979592	19.0740886264426\\
31.3734693877551	20.917789563099\\
31.414693877551	22.8059096330123\\
31.4559183673469	24.7244781741203\\
31.4971428571429	26.6196597723966\\
31.5383673469388	28.5169716481121\\
31.5795918367347	30.4618468879127\\
31.6208163265306	32.4286297223982\\
31.6620408163265	34.38459120871\\
31.7032653061225	36.3646379253621\\
31.7444897959184	38.4156758217423\\
31.7857142857143	40.5418260475369\\
31.8269387755102	42.7491697746657\\
31.8681632653061	45.0900878115108\\
31.909387755102	47.6932549511185\\
};
\addlegendentry{$t_i$, $I=25$}

\addplot [color=mycolor4, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
30.92	2.2877809782418\\
31.0024489795918	2.26977650369783\\
31.0848979591837	3.72295973855241\\
31.1673469387755	4.80686107685805\\
31.2497959183673	5.71067810104506\\
31.3322448979592	6.50771801208339\\
31.414693877551	7.09794636506338\\
31.4971428571429	7.77010385085785\\
31.5795918367347	8.47069831278414\\
31.6620408163265	9.25184997999163\\
31.7444897959184	10.1413419394341\\
31.8269387755102	11.3332432387678\\
31.909387755102	13.1357357616308\\
};
\addlegendentry{$t_i$, $I=13$}

\end{axis}

